Subtractive Training for Music Stem Insertion using Latent Diffusion Models

We present Subtractive Training, a simple and novel method for synthesizing individual musical instrument stems given other instruments as context. This method pairs a dataset of complete music mixes with 1) a variant of the dataset lacking a specific stem, and 2) LLM-generated instructions describing how the missing stem should be reintroduced. We then fine-tune a pretrained text-to-audio diffusion model to generate the missing instrument stem, guided by both the existing stems and the text instruction. Our results demonstrate Subtractive Training's efficacy in creating authentic drum stems that seamlessly blend with the existing tracks. We also show that we can use the text instruction to control the generation of the inserted stem in terms of rhythm, dynamics, and genre, allowing us to modify the style of a single instrument in a full song while keeping the remaining instruments the same. Lastly, we extend this technique to MIDI formats, successfully generating compatible bass, drum, and guitar parts for incomplete arrangements.

==> figs/midi_examples_2.tex <==
\begin{figure}[h]
  \centering
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0.2cm 0cm 0cm 0cm, clip]{figs/midi_examples/ExampleRoll_D_2163.pdf}
    \vspace{-15pt}
    \caption{Drum Generation}

  \end{subfigure}
  
  
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0.2cm 0cm 0cm 0cm, clip]{figs/midi_examples/ExampleRoll_B_.pdf}
    \vspace{-15pt}
    \caption{Bass Generation}

  \end{subfigure}
  
  
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth,trim=0.2cm 0cm 0cm 0cm, clip]{figs/midi_examples/ExampleRoll_G_0.pdf}
    \vspace{-15pt}
    \caption{Guitar Generation}

  \end{subfigure}

  \caption{Pitch rolls showing stem-generation results using three different diffusion models, each trained to output a given instrument. The notes corresponding to the generated instrument are outlined in black.}
  \label{fig:midi}
\end{figure}

